The Volume Capture in Structures with Variable Curvature

The volume capture in classical relativistic mechanics is considered as a scattering process for the high energy charged particles in a field with no central or mirror symmetry. The parameters of volume capture for potentials with smooth variable curvature are received and analyzed.

==> files/01_Classical.tex <==
\section{\label{sec:level1} Introduction}
It is well known that the symmetry of straight or bent crystal with constant curvature does not allow the volume capture of particles in the channels in Hamiltonian mechanics. In quantum mechanics, however, there is a possibility of the volume capture due to exponentially small tunneling effect through the potential barrier, but we will not consider it here. We also will not consider the incoherent scattering which causes the volume capture ~\cite{tar98,bck} and the normal dechanneling. The volume capture, as a pure classical effect, becomes possible due to curvature variation ('gradient capture') which was pointed out in the computer simulation /1/ and discussed in 80th -90th (see e.g.~\cite{tar98,bck}). Here we discussed some common features and relations of volume captures.
 
